NBR: Neutralization Based Reclamation

Safe memory reclamation (SMR) algorithms suffer from a trade-off between bounding unreclaimed memory and the speed of reclamation. Hazard pointer (HP) based algorithms bound unreclaimed memory at all times, but tend to be slower than other approaches. Epoch based reclamation (EBR) algorithms are faster, but do not bound memory reclamation. Other algorithms follow hybrid approaches, requiring special compiler or hardware support, changes to record layouts, and/or extensive code changes. Not all SMR algorithms can be used to reclaim memory for all data structures. We propose a new neutralization based reclamation (NBR) algorithm that is faster than the best known EBR algorithms and achieves bounded unreclaimed memory. It is non-blocking when used with a non-blocking operating system (OS) kernel, and only requires atomic read, write and CAS. NBR is straightforward to use with many different data structures, and in most cases, require similar reasoning and programmer effort to two-phased locking. NBR is implemented using OS signals and a lightweight handshaking mechanism between participating threads to determine when it is safe to reclaim a record. Experiments on a lock-based binary search tree and a lazy linked list show that NBR significantly outperforms many state of the art reclamation algorithms. In the tree NBR is faster than next best algorithm, DEBRA by upto 38% and HP by upto 17%. And, in the list NBR is 15% and 243% faster than DEBRA and HP, respectively.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle


==> figs/dsop3phase <==
\setlength{\unitlength}{4144sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(15330,3411)(1336,-4495)
\thinlines
{\color[rgb]{0,0,0}\multiput(4349,-2671)(-116.83871,0.00000){16}{\line(-1, 0){ 58.419}}
}%
{\color[rgb]{0,0,0}\multiput(14751,-2671)(115.33333,0.00000){17}{\line( 1, 0){ 57.667}}
}%
\thicklines
{\color[rgb]{0,0,0}\put(9271,-1861){\line( 0,-1){1784}}
}%
\thinlines
{\color[rgb]{0,0,0}\put(4456,-2671){\line( 1, 0){10170}}
}%
{\color[rgb]{0,0,0}\put(4996,-1816){\line( 1, 0){9000}}
}%
\thicklines
{\color[rgb]{0,0,0}\multiput(4407,-3391)(226.37209,0.00000){22}{\line( 1, 0){113.186}}
\put(9274,-3391){\vector( 1, 0){0}}
\put(4407,-3391){\vector(-1, 0){0}}
}%
{\color[rgb]{0,0,0}\multiput(9272,-3391)(225.91489,0.00000){24}{\line( 1, 0){112.957}}
\put(14581,-3391){\vector( 1, 0){0}}
\put(9272,-3391){\vector(-1, 0){0}}
}%
{\color[rgb]{0,0,0}\put(5042,-1631){\line(-1, 0){  2}}
\multiput(5035,-1632)(-9.89190,-1.64865){2}{\makebox(6.3500,9.5250){\small.}}
\multiput(5025,-1633)(-13.94590,-2.32432){2}{\makebox(6.3500,9.5250){\small.}}
\multiput(5011,-1635)(-9.48650,-1.58108){3}{\makebox(6.3500,9.5250){\small.}}
\multiput(4992,-1638)(-8.00000,-1.33333){4}{\makebox(6.3500,9.5250){\small.}}
\multiput(4968,-1642)(-9.67567,-1.61261){4}{\makebox(6.3500,9.5250){\small.}}
\multiput(4939,-1647)(-7.70587,-1.92647){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4908,-1654)(-8.70588,-2.17647){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4873,-1662)(-8.76470,-2.19117){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4838,-1671)(-8.92500,-2.97500){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4802,-1682)(-8.70000,-2.90000){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4767,-1693)(-8.44828,-3.37931){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4733,-1706)(-8.10345,-3.24138){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4701,-1720)(-7.60000,-3.80000){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4671,-1736)(-6.91177,-4.14706){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4643,-1752)(-6.44000,-4.83000){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4617,-1771)(-7.80327,-6.50272){4}{\makebox(6.3500,9.5250){\small.}}
\multiput(4594,-1791)(-7.16667,-7.16667){4}{\makebox(6.3500,9.5250){\small.}}
\multiput(4572,-1812)(-6.37400,-7.96750){4}{\makebox(6.3500,9.5250){\small.}}
\multiput(4553,-1836)(-5.84617,-8.76925){4}{\makebox(6.3500,9.5250){\small.}}
\multiput(4535,-1862)(-4.14705,-6.91175){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4519,-1890)(-3.85000,-7.70000){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4504,-1921)(-3.37930,-8.44825){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4491,-1955)(-3.07500,-9.22500){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4479,-1992)(-3.10000,-9.30000){4}{\makebox(6.3500,9.5250){\small.}}
\multiput(4470,-2020)(-2.50980,-10.03920){4}{\makebox(6.3500,9.5250){\small.}}
\multiput(4462,-2050)(-1.92647,-7.70590){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4455,-2081)(-1.65385,-8.26925){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4448,-2114)(-1.75000,-8.75000){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4441,-2149)(-1.50000,-9.00000){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4435,-2185)(-1.58108,-9.48645){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4429,-2223)(-1.61488,-9.68925){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4424,-2262)(-1.32432,-7.94592){6}{\makebox(6.3500,9.5250){\small.}}
\multiput(4419,-2302)(-1.38918,-8.33508){6}{\makebox(6.3500,9.5250){\small.}}
\multiput(4414,-2344)(-1.41622,-8.49732){6}{\makebox(6.3500,9.5250){\small.}}
\put(4410,-2387){\line( 0,-1){ 45}}
\put(4407,-2432){\line( 0,-1){ 45}}
\put(4404,-2477){\line( 0,-1){ 46}}
\put(4402,-2523){\line( 0,-1){ 47}}
\put(4400,-2570){\line( 0,-1){ 48}}
\put(4398,-2618){\line( 0,-1){ 47}}
\put(4398,-2665){\line( 0,-1){ 49}}
\put(4397,-2714){\line( 0,-1){ 48}}
\put(4398,-2762){\line( 0,-1){ 47}}
\put(4398,-2809){\line( 0,-1){ 48}}
\put(4400,-2857){\line( 0,-1){ 47}}
\put(4402,-2904){\line( 0,-1){ 46}}
\put(4404,-2950){\line( 0,-1){ 45}}
\put(4407,-2995){\line( 0,-1){ 45}}
\multiput(4410,-3040)(1.41622,-8.49732){6}{\makebox(6.3500,9.5250){\small.}}
\multiput(4414,-3083)(1.38918,-8.33508){6}{\makebox(6.3500,9.5250){\small.}}
\multiput(4419,-3125)(1.32432,-7.94592){6}{\makebox(6.3500,9.5250){\small.}}
\multiput(4424,-3165)(1.61488,-9.68925){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4429,-3204)(1.58108,-9.48645){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4435,-3242)(1.50000,-9.00000){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4441,-3278)(1.75000,-8.75000){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4448,-3313)(1.65385,-8.26925){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4455,-3346)(1.92647,-7.70590){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4462,-3377)(2.50980,-10.03920){4}{\makebox(6.3500,9.5250){\small.}}
\multiput(4470,-3407)(3.10000,-9.30000){4}{\makebox(6.3500,9.5250){\small.}}
\multiput(4479,-3435)(3.07500,-9.22500){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4491,-3472)(3.37930,-8.44825){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4504,-3506)(3.85000,-7.70000){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4519,-3537)(4.14705,-6.91175){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4535,-3565)(5.84617,-8.76925){4}{\makebox(6.3500,9.5250){\small.}}
\multiput(4553,-3591)(6.37400,-7.96750){4}{\makebox(6.3500,9.5250){\small.}}
\multiput(4572,-3615)(7.16667,-7.16667){4}{\makebox(6.3500,9.5250){\small.}}
\multiput(4594,-3636)(7.80327,-6.50272){4}{\makebox(6.3500,9.5250){\small.}}
\multiput(4617,-3656)(6.44000,-4.83000){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4643,-3675)(6.91177,-4.14706){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4671,-3691)(7.60000,-3.80000){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4701,-3707)(8.10345,-3.24138){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4733,-3721)(8.44828,-3.37931){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4767,-3734)(8.70000,-2.90000){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4802,-3745)(8.92500,-2.97500){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4838,-3756)(8.76470,-2.19117){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4873,-3765)(8.70588,-2.17647){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4908,-3773)(7.70587,-1.92647){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(4939,-3780)(9.67567,-1.61261){4}{\makebox(6.3500,9.5250){\small.}}
\multiput(4968,-3785)(8.00000,-1.33333){4}{\makebox(6.3500,9.5250){\small.}}
\multiput(4992,-3789)(9.48650,-1.58108){3}{\makebox(6.3500,9.5250){\small.}}
\multiput(5011,-3792)(13.94590,-2.32432){2}{\makebox(6.3500,9.5250){\small.}}
\multiput(5025,-3794)(9.89190,-1.64865){2}{\makebox(6.3500,9.5250){\small.}}
\put(5040,-3796){\line( 1, 0){  2}}
}%
{\color[rgb]{0,0,0}\put(14085,-3846){\line( 1, 0){  2}}
\multiput(14092,-3845)(9.89190,1.64865){2}{\makebox(6.3500,9.5250){\small.}}
\multiput(14102,-3844)(13.94590,2.32432){2}{\makebox(6.3500,9.5250){\small.}}
\multiput(14116,-3842)(9.48650,1.58108){3}{\makebox(6.3500,9.5250){\small.}}
\multiput(14135,-3839)(8.00000,1.33333){4}{\makebox(6.3500,9.5250){\small.}}
\multiput(14159,-3835)(9.67567,1.61261){4}{\makebox(6.3500,9.5250){\small.}}
\multiput(14188,-3830)(7.70587,1.92647){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14219,-3823)(8.70588,2.17647){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14254,-3815)(8.76470,2.19117){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14289,-3806)(8.92500,2.97500){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14325,-3795)(8.70000,2.90000){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14360,-3784)(8.44828,3.37931){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14394,-3771)(8.10345,3.24138){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14426,-3757)(7.60000,3.80000){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14456,-3741)(6.91177,4.14706){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14484,-3725)(6.44000,4.83000){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14510,-3706)(7.80327,6.50272){4}{\makebox(6.3500,9.5250){\small.}}
\multiput(14533,-3686)(7.16667,7.16667){4}{\makebox(6.3500,9.5250){\small.}}
\multiput(14555,-3665)(6.37400,7.96750){4}{\makebox(6.3500,9.5250){\small.}}
\multiput(14574,-3641)(5.84617,8.76925){4}{\makebox(6.3500,9.5250){\small.}}
\multiput(14592,-3615)(4.14705,6.91175){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14608,-3587)(3.85000,7.70000){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14623,-3556)(3.37930,8.44825){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14636,-3522)(3.07500,9.22500){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14648,-3485)(3.10000,9.30000){4}{\makebox(6.3500,9.5250){\small.}}
\multiput(14657,-3457)(2.50980,10.03920){4}{\makebox(6.3500,9.5250){\small.}}
\multiput(14665,-3427)(1.92647,7.70590){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14672,-3396)(1.65385,8.26925){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14679,-3363)(1.75000,8.75000){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14686,-3328)(1.50000,9.00000){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14692,-3292)(1.58108,9.48645){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14698,-3254)(1.61488,9.68925){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14703,-3215)(1.32432,7.94592){6}{\makebox(6.3500,9.5250){\small.}}
\multiput(14708,-3175)(1.38918,8.33508){6}{\makebox(6.3500,9.5250){\small.}}
\multiput(14713,-3133)(1.41622,8.49732){6}{\makebox(6.3500,9.5250){\small.}}
\put(14717,-3090){\line( 0, 1){ 45}}
\put(14720,-3045){\line( 0, 1){ 45}}
\put(14723,-3000){\line( 0, 1){ 46}}
\put(14725,-2954){\line( 0, 1){ 47}}
\put(14727,-2907){\line( 0, 1){ 48}}
\put(14729,-2859){\line( 0, 1){ 47}}
\put(14729,-2812){\line( 0, 1){ 49}}
\put(14730,-2763){\line( 0, 1){ 48}}
\put(14729,-2715){\line( 0, 1){ 47}}
\put(14729,-2668){\line( 0, 1){ 48}}
\put(14727,-2620){\line( 0, 1){ 47}}
\put(14725,-2573){\line( 0, 1){ 46}}
\put(14723,-2527){\line( 0, 1){ 45}}
\put(14720,-2482){\line( 0, 1){ 45}}
\multiput(14717,-2437)(-1.41622,8.49732){6}{\makebox(6.3500,9.5250){\small.}}
\multiput(14713,-2394)(-1.38918,8.33508){6}{\makebox(6.3500,9.5250){\small.}}
\multiput(14708,-2352)(-1.32432,7.94592){6}{\makebox(6.3500,9.5250){\small.}}
\multiput(14703,-2312)(-1.61488,9.68925){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14698,-2273)(-1.58108,9.48645){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14692,-2235)(-1.50000,9.00000){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14686,-2199)(-1.75000,8.75000){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14679,-2164)(-1.65385,8.26925){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14672,-2131)(-1.92647,7.70590){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14665,-2100)(-2.50980,10.03920){4}{\makebox(6.3500,9.5250){\small.}}
\multiput(14657,-2070)(-3.10000,9.30000){4}{\makebox(6.3500,9.5250){\small.}}
\multiput(14648,-2042)(-3.07500,9.22500){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14636,-2005)(-3.37930,8.44825){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14623,-1971)(-3.85000,7.70000){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14608,-1940)(-4.14705,6.91175){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14592,-1912)(-5.84617,8.76925){4}{\makebox(6.3500,9.5250){\small.}}
\multiput(14574,-1886)(-6.37400,7.96750){4}{\makebox(6.3500,9.5250){\small.}}
\multiput(14555,-1862)(-7.16667,7.16667){4}{\makebox(6.3500,9.5250){\small.}}
\multiput(14533,-1841)(-7.80327,6.50272){4}{\makebox(6.3500,9.5250){\small.}}
\multiput(14510,-1821)(-6.44000,4.83000){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14484,-1802)(-6.91177,4.14706){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14456,-1786)(-7.60000,3.80000){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14426,-1770)(-8.10345,3.24138){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14394,-1756)(-8.44828,3.37931){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14360,-1743)(-8.70000,2.90000){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14325,-1732)(-8.92500,2.97500){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14289,-1721)(-8.76470,2.19117){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14254,-1712)(-8.70588,2.17647){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14219,-1704)(-7.70587,1.92647){5}{\makebox(6.3500,9.5250){\small.}}
\multiput(14188,-1697)(-9.67567,1.61261){4}{\makebox(6.3500,9.5250){\small.}}
\multiput(14159,-1692)(-8.00000,1.33333){4}{\makebox(6.3500,9.5250){\small.}}
\multiput(14135,-1688)(-9.48650,1.58108){3}{\makebox(6.3500,9.5250){\small.}}
\multiput(14116,-1685)(-13.94590,2.32432){2}{\makebox(6.3500,9.5250){\small.}}
\multiput(14102,-1683)(-9.89190,1.64865){2}{\makebox(6.3500,9.5250){\small.}}
\put(14087,-1681){\line(-1, 0){  2}}
}%
\put(1351,-2401){\makebox(0,0)[lb]{\smash{{\SetFigFont{34}{40.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}Quiescent}%
}}}}
\put(2431,-3211){\makebox(0,0)[lb]{\smash{{\SetFigFont{34}{40.8}{\familydefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}phase}%
}}}}
\put(15031,-2401){\makebox(0,0)[lb]{\smash{{\SetFigFont{34}{40.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}Quiescent}%
}}}}
\put(15391,-3121){\makebox(0,0)[lb]{\smash{{\SetFigFont{34}{40.8}{\familydefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}phase}%
}}}}
\put(9631,-3211){\makebox(0,0)[lb]{\smash{{\SetFigFont{34}{40.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}non-neutralizable}%
}}}}
\put(5041,-3211){\makebox(0,0)[lb]{\smash{{\SetFigFont{34}{40.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}neutralizable}%
}}}}
\put(6211,-1591){\makebox(0,0)[lb]{\smash{{\SetFigFont{34}{40.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}data-structure operation}%
}}}}
\put(9001,-4291){\makebox(0,0)[lb]{\smash{{\SetFigFont{34}{40.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}begin$\Phi_{write}$}%
}}}}
\put(2881,-4291){\makebox(0,0)[lb]{\smash{{\SetFigFont{34}{40.8}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}begin$\Phi_{read}$}%
}}}}
\end{picture}%


==> figs/llex <==
\setlength{\unitlength}{4144sp}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\begin{picture}(7038,2803)(1570,-4553)
\thinlines
{\color[rgb]{0,0,0}\put(4567,-3376){\oval(390,390)[bl]}
\put(4567,-3091){\oval(390,390)[tl]}
\put(5611,-3376){\oval(390,390)[br]}
\put(5611,-3091){\oval(390,390)[tr]}
\put(4567,-3571){\line( 1, 0){1044}}
\put(4567,-2896){\line( 1, 0){1044}}
\put(4372,-3376){\line( 0, 1){285}}
\put(5806,-3376){\line( 0, 1){285}}
}%
{\color[rgb]{0,0,0}\put(7357,-3376){\oval(390,390)[bl]}
\put(7357,-3091){\oval(390,390)[tl]}
\put(8401,-3376){\oval(390,390)[br]}
\put(8401,-3091){\oval(390,390)[tr]}
\put(7357,-3571){\line( 1, 0){1044}}
\put(7357,-2896){\line( 1, 0){1044}}
\put(7162,-3376){\line( 0, 1){285}}
\put(8596,-3376){\line( 0, 1){285}}
}%
{\color[rgb]{0,0,0}\multiput(3016,-3211)(117.39130,0.00000){12}{\line( 1, 0){ 58.696}}
\put(4366,-3211){\vector( 1, 0){0}}
}%
{\color[rgb]{0,0,0}\put(4636,-1906){\vector( 0,-1){1035}}
}%
{\color[rgb]{0,0,0}\put(1777,-3421){\oval(390,390)[bl]}
\put(1777,-3136){\oval(390,390)[tl]}
\put(2821,-3421){\oval(390,390)[br]}
\put(2821,-3136){\oval(390,390)[tr]}
\put(1777,-3616){\line( 1, 0){1044}}
\put(1777,-2941){\line( 1, 0){1044}}
\put(1582,-3421){\line( 0, 1){285}}
\put(3016,-3421){\line( 0, 1){285}}
}%
{\color[rgb]{0,0,0}\put(5806,-3211){\vector( 1, 0){1350}}
}%
{\color[rgb]{0,0,0}\multiput(3040,-3325)(9.90000,-3.30000){2}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(3050,-3328)(15.00000,-5.00000){2}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(3065,-3333)(9.39655,-3.75862){3}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(3084,-3340)(8.00000,-2.66667){4}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(3108,-3348)(10.00000,-3.33333){4}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(3138,-3358)(8.77500,-2.92500){5}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(3173,-3370)(8.16000,-2.72000){6}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(3214,-3383)(7.65000,-2.55000){7}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(3260,-3398)(8.50000,-2.83333){7}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(3311,-3415)(7.71429,-2.57143){8}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(3365,-3433)(8.40000,-2.80000){8}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(3424,-3452)(7.57500,-2.52500){9}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(3485,-3471)(7.95000,-2.65000){9}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(3549,-3491)(8.10000,-2.70000){9}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(3614,-3512)(8.28750,-2.76250){9}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(3681,-3532)(8.32500,-2.77500){9}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(3748,-3553)(8.28750,-2.76250){9}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(3815,-3573)(8.32353,-2.08088){9}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(3881,-3592)(8.32353,-2.08088){9}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(3947,-3611)(8.17647,-2.04412){9}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(4012,-3629)(7.94118,-1.98529){9}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(4075,-3647)(8.73950,-2.18487){8}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(4136,-3663)(8.57143,-2.14286){8}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(4196,-3678)(8.43697,-2.10924){8}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(4255,-3693)(7.96639,-1.99160){8}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(4311,-3706)(7.83193,-1.95798){8}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(4366,-3719)(8.84615,-1.76923){7}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(4419,-3730)(8.68590,-1.73718){7}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(4471,-3741)(8.35135,-1.39189){7}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(4521,-3750)(8.00000,-1.33333){7}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(4569,-3758)(8.00000,-1.33333){7}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(4617,-3766)(9.34054,-1.55676){6}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(4664,-3772)(8.95136,-1.49189){6}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(4709,-3778)(8.91892,-1.48649){6}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(4754,-3783)(8.69190,-1.44865){6}{\makebox(1.5875,11.1125){\tiny.}}
\put(4798,-3787){\line( 1, 0){ 44}}
\put(4842,-3790){\line( 1, 0){ 44}}
\put(4886,-3792){\line( 1, 0){ 44}}
\put(4930,-3793){\line( 1, 0){ 43}}
\put(4973,-3794){\line( 1, 0){ 44}}
\put(5017,-3794){\line( 1, 0){ 41}}
\put(5058,-3793){\line( 1, 0){ 42}}
\put(5100,-3791){\line( 1, 0){ 43}}
\put(5143,-3789){\line( 1, 0){ 42}}
\put(5185,-3786){\line( 1, 0){ 44}}
\multiput(5229,-3783)(8.72432,1.45405){6}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(5273,-3778)(8.72432,1.45405){6}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(5317,-3773)(9.14594,1.52432){6}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(5363,-3767)(9.37298,1.56216){6}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(5410,-3760)(8.00000,1.33333){7}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(5458,-3752)(8.32432,1.38739){7}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(5508,-3744)(8.49358,1.69872){7}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(5559,-3734)(8.81410,1.76282){7}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(5612,-3724)(9.03847,1.80769){7}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(5666,-3712)(8.15934,1.63187){8}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(5723,-3700)(8.26891,2.06723){8}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(5781,-3686)(8.53781,2.13445){8}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(5841,-3672)(7.85294,1.96323){9}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(5904,-3657)(8.02941,2.00735){9}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(5968,-3640)(8.26470,2.06617){9}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(6034,-3623)(8.52941,2.13235){9}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(6102,-3605)(7.81699,1.95425){10}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(6172,-3586)(7.81699,1.95425){10}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(6242,-3567)(8.05229,2.01307){10}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(6314,-3547)(8.18301,2.04575){10}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(6387,-3526)(8.18301,2.04575){10}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(6460,-3505)(7.90000,2.63333){10}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(6532,-3484)(7.80000,2.60000){10}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(6603,-3463)(7.70000,2.56667){10}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(6673,-3442)(8.40000,2.80000){9}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(6741,-3422)(8.06250,2.68750){9}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(6806,-3402)(7.53750,2.51250){9}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(6867,-3384)(8.22857,2.74286){8}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(6925,-3366)(8.60000,2.86667){7}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(6977,-3350)(7.95000,2.65000){7}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(7025,-3335)(8.16000,2.72000){6}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(7066,-3322)(9.15000,3.05000){5}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(7103,-3311)(10.00000,3.33333){4}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(7133,-3301)(8.39217,2.09804){4}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(7158,-3294)(10.05000,3.35000){3}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(7178,-3287)(15.05880,3.76470){2}{\makebox(1.5875,11.1125){\tiny.}}
\multiput(7193,-3283)(10.50000,3.50000){3}{\makebox(1.5875,11.1125){\tiny.}}
\put(7214,-3276){\vector( 3, 1){0}}
}%
\put(1666,-3391){\makebox(0,0)[lb]{\smash{{\SetFigFont{20}{24.0}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$rec_1$}%
}}}}
\put(1666,-3391){\makebox(0,0)[lb]{\smash{{\SetFigFont{20}{24.0}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$rec_1$}%
}}}}
\put(4411,-3346){\makebox(0,0)[lb]{\smash{{\SetFigFont{20}{24.0}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$rec_2$}%
}}}}
\put(7246,-3346){\makebox(0,0)[lb]{\smash{{\SetFigFont{20}{24.0}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$rec_3$}%
}}}}
\put(4771,-2761){\makebox(0,0)[lb]{\smash{{\SetFigFont{20}{24.0}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}(iv):$curr.next$}%
}}}}
\put(4771,-2356){\makebox(0,0)[lb]{\smash{{\SetFigFont{20}{24.0}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}(i):$curr=rec_1.next$}%
}}}}
\put(4636,-2041){\makebox(0,0)[lb]{\smash{{\SetFigFont{20}{24.0}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$T_s$}%
}}}}
\put(3466,-4066){\makebox(0,0)[lb]{\smash{{\SetFigFont{20}{24.0}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}(ii):$rec_1.next=rec_3$}%
}}}}
\put(3511,-4426){\makebox(0,0)[lb]{\smash{{\SetFigFont{20}{24.0}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}(iii):$free(rec_2)$}%
}}}}
\put(3196,-3751){\makebox(0,0)[lb]{\smash{{\SetFigFont{20}{24.0}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$T_r$}%
}}}}
\put(7021,-2851){\makebox(0,0)[lb]{\smash{{\SetFigFont{20}{24.0}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}\textcolor{red}{\xmark}}%
}}}}
\end{picture}%


==> sections/abstract.tex <==
\begin{abstract}
\iffalse
A \textit{safe memory reclamation} (SMR) algorithm %for concurrent data structures 
determines when is it safe to reclaim a shared record that has been unlinked from a concurrent data structure.
Existing SMR algorithms lack various properties that are desirable in concurrent data structures. %property to be practically useful in concurrent data structures.
For example, hazard pointer (HP) based algorithms are \emph{robust}, meaning the amount of unreclaimed garbage is bounded at all times, even if some threads can experience \textit{halting failures}, but they are not as \emph{fast} as %quiescent state based and 
epoch based reclamation (EBR).
On the other hand, EBR is \emph{fast}, but not \emph{robust}.
Some reference counting based algorithms are neither \emph{fast} nor \emph{robust}.
Other algorithms follow hybrid approaches, requiring special compiler or hardware support, changes to record layouts, and/or extensive code changes. % like, hardware transaction memory or primitives like double word CAS.
There is also the question of \textit{applicability}: not all SMR algorithms can be used to reclaim memory for all data structures.
% Moreover, some SMR algorithms are fast only under very specific workloads, whereas consistent performance across a wide range of workloads is often desirable.

% Similarly, other hybrid approaches are intrusive.
% Firstly, in a way that requires changes to data structure records to maintain metadata (eg., Hazard Eras and IBR require storing birth-era alongside records) or may require to use customized allocation for records (like Free Access).
% Secondly, in a way that may force programmers to use per read fence and validation (eg, Hazard pointers and Lock-free reference counting).
% Thus, increasing programming effort.

% While there are others that apply to a limited class of data structures. For example, DEBRA+ which could not be applied to optimistic lock-based data structures. Furthermore, there are some which perform well on workloads of certain characteristics only, like reference counting do not scale well for update intensive workloads and there are others which scale badly with over-subscription (eg, EBR). Thus, balancing \emph{speed}, \emph{robustness}, \emph{usability}, \emph{transparency} and \emph{wide applicability} has been a challenge for \smr. 

We propose a new \textit{neutralization} based reclamation (NBR) algorithm which is robust, yet faster than DEBRA, the best-known epoch based reclamation algorithm.
It is non-blocking when used with a non-blocking operating system (OS) kernel, and only requires atomic read, write and CAS.
NBR is straightforward to use with many data structures, requiring similar reasoning (and programming effort) to two-phased locking. %requiring similar reasoning to two-phased locking. %provides qualitative advantages of better usability\textendash as it has an 
%interface is similar as simple to use as using locks in terms of programming effort, has wide applicability \textendash as \nbr does not require any special compiler support or hardware mechanisms and do not assume any workload characteristics.
\nbr is implemented using OS signals and a lightweight handshaking mechanism between participating threads to determine when it is safe to reclaim a record.

Experiments on a lock-based binary search tree and a lazy linked list show that \nbr significantly outperforms many state of the art reclamation algorithms.
For example, NBR outperforms the next fastest algorithm, DEBRA, by up to 38\% in the tree and 29\% in the list, and outperforms HP by up to 32\% in the tree and 234\% in the list.

% As a further optimization, we use the Dune system, which provides applications with the ability to use to privileged CPU features to improve performance through direct use of inter-processor interrupts as a faster replacement to POSIX signals.

%
%Our experiments show that \nbr significantly outperforms the state of the art in many workloads and maintains good performance even when there are long thread delays, or many more threads than cores. %, and reclamation workload is evenly balanced across all threads.
%Thus, given its qualitative advantages, \nbr could be a good alternative to achieve \smr in concurrent data structure libraries.

new:
\fi

\textit{Safe memory reclamation} (SMR) algorithms suffer from a trade-off between bounding unreclaimed memory and the speed of reclamation.
Hazard pointer (HP) based algorithms bound unreclaimed memory at all times, but tend to be slower than other approaches.
Epoch based reclamation (EBR) algorithms are faster, but do not bound memory reclamation.
Other algorithms follow hybrid approaches, requiring special compiler or hardware support, changes to record layouts, and/or extensive code changes.
Not all SMR algorithms can be used to reclaim memory for all data structures.

We propose a new \textit{neutralization} based reclamation (NBR) algorithm that achieves both bounded reclamation and faster than the best known EBR algorithms.
It is non-blocking when used with a non-blocking operating system (OS) kernel, and only requires atomic read, write and CAS.
NBR is straightforward to use with many different data structures, requiring similar reasoning and programmer effort to two-phased locking.
\nbr is implemented using OS signals and a lightweight handshaking mechanism between participating threads to determine when it is safe to reclaim a record.
Experiments on a lock-based binary search tree and a lazy linked list show that \nbr significantly outperforms many state of the art reclamation algorithms.
NBR outperforms the next fastest algorithm, DEBRA, by up to 26\% in the tree and 30\% in the list, and outperforms HP by up to 22\% (tree) and 247\% (list).

% %As a faster alternative to POSIX signals, and to acheive non-blocking progress,
% We also explore the use of the Dune system, which provides applications with the ability to use to privileged CPU features, to improve performance and achieve non-blocking progress through direct use of inter-processor interrupts. % as a faster replacement to POSIX signals.
% %Additionally, whereas signals are blocking in the Linux kernel, Dune's non-blocking IPIs allow us to 
% %Dune's IPIs are also non-blocking, which allows 

\end{abstract}


==> sections/misc.tex <==
\ignore{

\section{REMOVEMEATLAST Misc:NBR strengths}\XXX{REMOVE MEAT LAST? :p}
\begin{enumerate}
    \item [app] NBR unlike HP, doesn't have deleted-node traversal pathology first mentioned by Debra and then by cohen \cite{cohen2018every} in 2018. Thus, NBR applies well to data structures where deleted nodes are allowed to traverse to have more efficient lokups.
    \item [applicability] NBR applies to lockbased non blocking data structures as well like lazylist. Debra plus doesn't as it is risky to neutralize a process while it holds a lock. 
    \item June 4 Meeting ~1:10 in Video rec.  oversubscription + Pinning is experimental mistake : most of the time is spent in measuring system : cpu utilization is worse as lot of cpus are idle.  A section about this in paper. 
    \item while you talk about reader writer handshake.. through example say a list and illustrate how two nodes deleted crash pathology won't occur (DEBRA).. and how bcse op readers handshake its correct to access any node reachable from saved pointers---> wait no dereferencing any node is incorrect.. hmm see Cohen paper for the example and try to fit in your handshake illustration that how these problems are fixed. purpose is that read will be able to appreciate the illustrations of kind of challenges which NBR fixes and will also make them feel good that they learned some pedagogical info.  
    \item Fraser's EBR variant advances a epoch once each thread has announced the current epoch. While QSBR based EBR allows reclamation once each thread has been through a Quiescent period[from IBR paper].
    
    \item[app] harris list and harris-herlihy-shavit list are not compatible with HP because of logically deleted nodes traversal phenomenon... two consecutive node deleted and first protected therefore second can be accessed and reclaimed at same time.. causing crash.. (PEBR uses this pathology to fix in their proposed technique). I to shall mention this as an advantage... to talk about applicability.    Wlak through how neutralization will fix this... lucid example..

% may  wrong what they mean by imposes requiremenet.. Do they mean that their approach fixes it?PEBR imposes the second re-quirement for retirement: in essence, a retired block (e.g., the first node) should not be traversed to create a new local pointer (e.g., the second node) in a new active state. Why then PEBR claims that it satisfies all requirements at same time... use this to my advantage to claim that NBR is first.

    \item refer to my notebook notes, free access and PEBR both have similar ejecting mechanims... both use dirty flag kind flag... PEBR also has per acces HP protection overhead.. where publishing is only done on ejection..
    
    \item PEBR doesnt even beat EBR and they donot compare with any other SMR thus cannt claim to be fastest. Thus I can claim to be forst on all aspects of SMR.
    
    \item like blellochs recent technique NBR also has O(1) announcement time, O(1) retirement time.Include this in my discussion. Wait do we?
\end{enumerate}
}
